Adjusting the Ground Truth Annotations for Connectivity-Based Learning to Delineate

Deep learning-based approaches to delineating 3D structure depend on accurate annotations to train the networks. Yet, in practice, people, no matter how conscientious, have trouble precisely delineating in 3D and on a large scale, in part because the data is often hard to interpret visually and in part because the 3D interfaces are awkward to use. In this paper, we introduce a method that explicitly accounts for annotation inaccuracies. To this end, we treat the annotations as active contour models that can deform themselves while preserving their topology. This enables us to jointly train the network and correct potential errors in the original annotations. The result is an approach that boosts performance of deep networks trained with potentially inaccurate annotations. Code has been released at https://github.com/doruk-oner/AdjustingAnnotationswithSnakes.

==> fig/slack_effect.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}[ht!]
	\setlength{\tabcolsep}{1pt}
	\centering
	\begin{tabular}{cc} 
		\includegraphics[width=0.98\columnwidth]{fig/qual_slack2} &
	\end{tabular}
%	\vspace{-2mm}
	\caption{ {\bf Effect of Distance {\it d} on \CCQ{}.}
		\label{fig:slack_effect}
	}
\end{figure}


==> fig/visual.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure*}[!htb]
\centering
\begin{tabular}{ccccc} %{@{} c >{\centering\arraybackslash}m{0.18\textwidth}>{\centering\arraybackslash}m{0.18\textwidth} >{\centering\arraybackslash}m{0.18\textwidth} >{\centering\arraybackslash}m{0.18\textwidth} >{\centering\arraybackslash}m{0.18\textwidth} @{}}
& input & \baseline{} & \snakeSimple{} & \snakeFast{} & \snakeFull{} \\
\multirow{10}{*}{\rotatebox[origin=rb]{90}{\neurons{}}} &
\includegraphics[width=0.18\textwidth]{brain_im} &
\includegraphics[width=0.18\textwidth]{brain_unet_mse} &
\includegraphics[width=0.18\textwidth]{brain_unet_simp} &
\includegraphics[width=0.18\textwidth]{brain_unet_fast} &
\includegraphics[width=0.18\textwidth]{brain_unet_full} \\
&
\includegraphics[width=0.18\textwidth]{brain_im2} &
\includegraphics[width=0.18\textwidth]{brain_unet_mse2} &
\includegraphics[width=0.18\textwidth]{brain_unet_simp2} &
\includegraphics[width=0.18\textwidth]{brain_unet_fast2} &
\includegraphics[width=0.18\textwidth]{brain_unet_full2} \\
\\[-2mm]
\multirow{10}{*}{\rotatebox[origin=rb]{90}{\neuronsmisal{}}} &
\includegraphics[width=0.18\textwidth]{tabea_im} &
\includegraphics[width=0.18\textwidth]{tabea_unet_mse} &
\includegraphics[width=0.18\textwidth]{tabea_unet_simp} &
\includegraphics[width=0.18\textwidth]{tabea_unet_fast} &
\includegraphics[width=0.18\textwidth]{tabea_unet_full} \\
&
\includegraphics[width=0.18\textwidth]{tabea_im2} &
\includegraphics[width=0.18\textwidth]{tabea_unet_mse2} &
\includegraphics[width=0.18\textwidth]{tabea_unet_simp2} &
\includegraphics[width=0.18\textwidth]{tabea_unet_fast2} &
\includegraphics[width=0.18\textwidth]{tabea_unet_full2} \\
\end{tabular}
\caption{ \scriptsize {\bf Qualitative results using the \UNet{} architecture}. The green ellipses denote areas where \baseline{} generate unwarranted breaks in the delineations whereas \SnakeFull{} and 
\SnakeFast{} do not.
}
\label{fig:visual} 
\end{figure*}



==> fig/visual_brain.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure*}[!htb]
\centering
\begin{tabular}{@{} c >{\centering\arraybackslash}m{0.18\textwidth}>{\centering\arraybackslash}m{0.18\textwidth} >{\centering\arraybackslash}m{0.18\textwidth} >{\centering\arraybackslash}m{0.18\textwidth} >{\centering\arraybackslash}m{0.18\textwidth} @{}}
& input & \baseline{} & \snakeSimple{} & \snakeFast{} & \snakeFull{} \\
\multirow{10}{*}{\rotatebox[origin=rb]{90}{\UNet{}}} &
\includegraphics[width=0.18\textwidth]{brain_im} &
\includegraphics[width=0.18\textwidth]{brain_unet_mse} &
\includegraphics[width=0.18\textwidth]{brain_unet_simp} &
\includegraphics[width=0.18\textwidth]{brain_unet_fast} &
\includegraphics[width=0.18\textwidth]{brain_unet_full} \\
&
\includegraphics[width=0.18\textwidth]{brain_im2} &
\includegraphics[width=0.18\textwidth]{brain_unet_mse2} &
\includegraphics[width=0.18\textwidth]{brain_unet_simp2} &
\includegraphics[width=0.18\textwidth]{brain_unet_fast2} &
\includegraphics[width=0.18\textwidth]{brain_unet_full2} \\
\\[-2mm]
\multirow{10}{*}{\rotatebox[origin=rb]{90}{\DRU{}}} &
\includegraphics[width=0.18\textwidth]{brain_wei_im} &
\includegraphics[width=0.18\textwidth]{brain_wei_mse} &
\includegraphics[width=0.18\textwidth]{brain_wei_simp} &
\includegraphics[width=0.18\textwidth]{brain_wei_fast} &
\includegraphics[width=0.18\textwidth]{brain_wei_full} \\
&
\includegraphics[width=0.18\textwidth]{brain_wei_im2} &
\includegraphics[width=0.18\textwidth]{brain_wei_mse2} &
\includegraphics[width=0.18\textwidth]{brain_wei_simp2} &
\includegraphics[width=0.18\textwidth]{brain_wei_fast2} &
\includegraphics[width=0.18\textwidth]{brain_wei_full2} \\
\end{tabular}
\caption{ \label{fig:visual_brain}
Qualitative comparison of the test results on the \neurons{} data set. The green ellipses denote areas where training with the original annotations results in unwarranted breaks in the delineations at test time whereas our approach does not.
}
\end{figure*}



==> fig/visual_misaligned.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure*}[!htb]
\centering
\begin{tabular}{@{} c >{\centering\arraybackslash}m{0.18\textwidth}>{\centering\arraybackslash}m{0.18\textwidth} >{\centering\arraybackslash}m{0.18\textwidth} >{\centering\arraybackslash}m{0.18\textwidth} >{\centering\arraybackslash}m{0.18\textwidth} @{}}
& input & \baseline{} & \snakeSimple{} & \snakeFast{} & \snakeFull{} \\
 \multirow{10}{*}{\rotatebox[origin=rb]{90}{\UNet{}}} &
\includegraphics[width=0.18\textwidth]{tabea_im} &
\includegraphics[width=0.18\textwidth]{tabea_unet_mse} &
\includegraphics[width=0.18\textwidth]{tabea_unet_simp} &
\includegraphics[width=0.18\textwidth]{tabea_unet_fast} &
\includegraphics[width=0.18\textwidth]{tabea_unet_full} \\
&
\includegraphics[width=0.18\textwidth]{tabea_im2} &
\includegraphics[width=0.18\textwidth]{tabea_unet_mse2} &
\includegraphics[width=0.18\textwidth]{tabea_unet_simp2} &
\includegraphics[width=0.18\textwidth]{tabea_unet_fast2} &
\includegraphics[width=0.18\textwidth]{tabea_unet_full2} \\
\\[-2mm]
 \multirow{10}{*}{\rotatebox[origin=rb]{90}{\DRU{}}} &
 \includegraphics[width=0.18\textwidth]{tabea_wei_im} &
 \includegraphics[width=0.18\textwidth]{tabea_wei_mse} &
 \includegraphics[width=0.18\textwidth]{tabea_wei_simp} &
 \includegraphics[width=0.18\textwidth]{tabea_wei_fast} &
 \includegraphics[width=0.18\textwidth]{tabea_wei_full} \\
 &
 \includegraphics[width=0.18\textwidth]{tabea_wei_im2} &
 \includegraphics[width=0.18\textwidth]{tabea_wei_mse2} &
 \includegraphics[width=0.18\textwidth]{tabea_wei_simp2} &
 \includegraphics[width=0.18\textwidth]{tabea_wei_fast2} &
 \includegraphics[width=0.18\textwidth]{tabea_wei_full2} \\
\end{tabular}
\caption{ \label{fig:visual_misaligned}
Qualitative comparison of the test results on the \neuronsmisal{} data set. The green ellipses denote areas where training with the original annotations results in unwarranted breaks in the delineations at test time whereas our approach does not.
}
\end{figure*}



==> fig/visual_mra.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure*}[!htb]
\centering
\begin{tabular}{@{} c >{\centering\arraybackslash}m{0.18\textwidth}>{\centering\arraybackslash}m{0.18\textwidth} >{\centering\arraybackslash}m{0.18\textwidth} >{\centering\arraybackslash}m{0.18\textwidth} >{\centering\arraybackslash}m{0.18\textwidth} @{}}
& input & \baseline{} & \snakeSimple{} & \snakeFast{} & \snakeFull{} \\
 \multirow{10}{*}{\rotatebox[origin=rb]{90}{\UNet{}}} &
\includegraphics[width=0.18\textwidth]{mra_im} &
\includegraphics[width=0.18\textwidth]{mra_unet_mse} &
\includegraphics[width=0.18\textwidth]{mra_unet_simp} &
\includegraphics[width=0.18\textwidth]{mra_unet_fast} &
\includegraphics[width=0.18\textwidth]{mra_unet_full} \\
&
\includegraphics[width=0.18\textwidth]{mra_im2} &
\includegraphics[width=0.18\textwidth]{mra_unet_mse2} &
\includegraphics[width=0.18\textwidth]{mra_unet_simp2} &
\includegraphics[width=0.18\textwidth]{mra_unet_fast2} &
\includegraphics[width=0.18\textwidth]{mra_unet_full2} \\
\\[-2mm]
 \multirow{10}{*}{\rotatebox[origin=rb]{90}{\DRU{}}} &
\includegraphics[width=0.18\textwidth]{mra_wei_im} &
\includegraphics[width=0.18\textwidth]{mra_wei_mse} &
\includegraphics[width=0.18\textwidth]{mra_wei_simp} &
\includegraphics[width=0.18\textwidth]{mra_wei_fast} &
\includegraphics[width=0.18\textwidth]{mra_wei_full} \\
&
\includegraphics[width=0.18\textwidth]{mra_wei_im2} &
\includegraphics[width=0.18\textwidth]{mra_wei_mse2} &
\includegraphics[width=0.18\textwidth]{mra_wei_simp2} &
\includegraphics[width=0.18\textwidth]{mra_wei_fast2} &
\includegraphics[width=0.18\textwidth]{mra_wei_full2} \\
\end{tabular}
\caption{ \label{fig:visual_mra}
Qualitative comparison of the test results on the \mra{} data set. The green ellipses denote areas where training with the original annotations results in unwarranted breaks in the delineations at test time whereas our approach does not.
}
\end{figure*}



==> fig/visual_noise.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}[!htb]
	\centering
	\begin{tabular}{@{} c >{\centering\arraybackslash}m{0.3\columnwidth}>{\centering\arraybackslash}m{0.3\columnwidth} >{\centering\arraybackslash}m{0.3\columnwidth}  @{}}
		& input & \baseline{} & \snakeFast{} \\
		\multirow{1}{*}{\rotatebox[origin=c]{90}{\it Level 1}} &
		\includegraphics[width=0.3\columnwidth]{noise_im1} &
		\includegraphics[width=0.3\columnwidth]{noise_mse1} &
		\includegraphics[width=0.3\columnwidth]{noise_fast1} \\
		\\
		\multirow{1}{*}{\rotatebox[origin=c]{90}{\it Level 2}} &
		\includegraphics[width=0.3\columnwidth]{noise_im2} &
		\includegraphics[width=0.3\columnwidth]{noise_mse2} &
		\includegraphics[width=0.3\columnwidth]{noise_fast2} \\
		\\
		\multirow{1}{*}{\rotatebox[origin=c]{90}{\it Level 3}} &
		\includegraphics[width=0.3\columnwidth]{noise_im3} &
		\includegraphics[width=0.3\columnwidth]{noise_mse3} &
		\includegraphics[width=0.3\columnwidth]{noise_fast3} \\
	\end{tabular}
	\caption{ \label{fig:visual_noise}
		Qualitative comparison of the test results on the \neurons{} data set with different levels of annotation noise. The green ellipses denote areas where training with the original annotations results in unwarranted breaks in the delineations at test time whereas our approach does not.
	}
\end{figure}



==> fig/visual_sota.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure*}[!htb]
\centering
\begin{tabular}{@{} c >{\centering\arraybackslash}m{0.18\textwidth}>{\centering\arraybackslash}m{0.18\textwidth} >{\centering\arraybackslash}m{0.18\textwidth} >{\centering\arraybackslash}m{0.18\textwidth} >{\centering\arraybackslash}m{0.18\textwidth} @{}}
& input & \COPLE{} & \QAM{} & \DS{} & \snakeFull{} \\
\multirow{1}{*}{\rotatebox[origin=lm]{90}{\neurons{}}} &
\includegraphics[width=0.18\textwidth]{sota_brain_im} &
\includegraphics[width=0.18\textwidth]{sota_brain_dice} &
\includegraphics[width=0.18\textwidth]{sota_brain_qam} &
\includegraphics[width=0.18\textwidth]{sota_brain_ds6} &
\includegraphics[width=0.18\textwidth]{sota_brain_fast} \\
\\[-2mm]
\multirow{2}{*}{\rotatebox[origin=c]{90}{\neuronsmisal{}}} &
\includegraphics[width=0.18\textwidth]{sota_tabea_im} &
\includegraphics[width=0.18\textwidth]{sota_tabea_dice} &
\includegraphics[width=0.18\textwidth]{sota_tabea_qam} &
\includegraphics[width=0.18\textwidth]{sota_tabea_ds6} &
\includegraphics[width=0.18\textwidth]{sota_tabea_fast} \\

\end{tabular}
\caption{ \label{fig:visual_sota}
Qualitative comparison of the test results on the \neurons{} data set. The green ellipses denote areas where baselines result in unwarranted breaks in the delineations at test time whereas our approach does not.
}
\end{figure*}



==> tables/results.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{table}
\setlength{\tabcolsep}{3pt}
\center
\begin{tabular}{@{}l l  c c c  c c c  c  c c @{}}
\cmidrule{3-10}
 & & \multicolumn{3}{c}{Pixel-wise} & &  \multicolumn{2}{c}{Topology-aware} & & iter.\ t.\\
\cmidrule{3-5}
\cmidrule{7-8}
\cmidrule{10-10}
Dataset &  Method & Corr. & Compl.  & Qual.&   &APLS & TLTS & & s\\
\cmidrule{1-10}
\multirow{4}{*}{\neurons}
&\baseline{}   &     98.9 &     91.3 &     90.4 &&     80.3 &     80.9 && 2.8 \\ 
&\snakeSimple{}&     98.4 &     92.5 &     91.2 &&     84.2 &     83.4 && 3.8 \\
&\snakeFast{}  &{\bf 99.1}&     92.4 &{\bf 91.5} &&{\bf 89.5}&{\bf 84.9}&& 5.2 \\
&\snakeFull{}  &     98.8 &{\bf 92.6}&{\bf 91.5}&&     89.3 &{\bf 84.9}&& 18.9\\
\cmidrule{1-10}

\multirow{4}{*}{\neuronsmisal{}}
&\baseline{}       &     81.8     &     83.5     &     70.4     &&     65.8     &     63.6     && 2.8 \\ 
&\snakeSimple{}&     83.0     &     83.9     &     71.6     &&     70.4     &     68.8     && 3.4\\
&\snakeFast{}    &     83.1     & {\bf 85.5} &     72.9     &&     73.9     & {\bf 70.2} && 4.9\\
&\snakeFull{}     & {\bf 83.5} &     85.4     & {\bf 73.1} && {\bf 74.2} &    69.9      && 17.8\\
\cmidrule{1-10}

\multirow{4}{*}{\mra{}}
&\baseline{}       &     90.1     &     72.2     &     66.9     &&     49.8    &    50.4      && 2.8 \\ 
&\snakeSimple{}&     89.9     &     73.1      &     67.5     &&     53.5    &    53.1      && 3.7\\
&\snakeFast{}    & {\bf 90.3} & {\bf 73.5} &  {\bf 68.1} && {\bf 55.4} & {\bf 55.2} && 5.1\\
&\snakeFull{}     &       -        &       -        &       -        &&       -        &       -        && 18.5\\
\cmidrule{1-10}
\end{tabular}
\vspace{2mm}
\caption{
Performance of \UNet{} trained using Mean Squared Error \baseline{} and the proposed losses.
See section~\ref{subs:results} for a description.
 \label{tab:combined}
}
 \vspace{-3mm}
\end{table}


==> tables/results_brain.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{table}
\caption{
Performance of deep nets trained with different loss functions on the \neurons{} data set and the time needed for single training iteration.
%See section~\ref{subs:results} for description.
 \label{tab:results_brain}
}
\setlength{\tabcolsep}{3pt}
\center
\begin{tabular}{@{}l l  c c c  c c c  c  c c @{}}
\cmidrule{3-10}
 & & \multicolumn{3}{c}{Pixel-wise} & &  \multicolumn{2}{c}{Topology-aware} & & iter.\ t.\\
\cmidrule{3-5}
\cmidrule{7-8}
\cmidrule{10-10}
Arch. &  Method & Corr. & Compl.  & Qual.&   &APLS & TLTS & & s\\
\cmidrule{1-10}
\multirow{4}{*}{\UNet{}}
&\baseline{}   &     98.9 &     91.3 &     90.4 &&     80.3 &     80.9 && 2.8 \\ 
&\snakeSimple{}&     98.4 &     92.5 &     91.2 &&     84.2 &     83.4 && 3.8 \\
&\snakeFast{}  &        98.7     &  {\bf 95.0} &{\bf 93.8} &&{\bf 91.1}&{\bf 85.9}&& 5.2 \\
&\snakeFull{}  &     {\bf 99.0} &    94.4      & 93.5&&     89.3 &{\bf 85.9}&& 18.9\\
\cmidrule{1-10}
\multirow{4}{*}{\DRU{}}
&\baseline{}   &     97.2 &     94.0 &     91.5 &&     84.3 &     83.9 && 2.7 \\ 
&\snakeSimple{}& {\bf 97.4} &     95.2 &     92.9 &&     90.8 &     85.9 && 3.8 \\
&\snakeFast{}  &   97.0   &     {\bf 97.1} & {\bf 94.2} && 91.7& 88.1&& 5.3 \\
&\snakeFull{}  &     96.9 & 96.9& 94.1 && {\bf 91.8} &{\bf 89.3}&& 19.1\\
\cmidrule{1-10}
\end{tabular}
\end{table}


==> tables/results_dru.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{table}
\setlength{\tabcolsep}{3pt}
\center
\begin{tabular}{@{}l l  c c c  c c c  c  c c @{}}
\cmidrule{3-10}
 & & \multicolumn{3}{c}{Pixel-wise} & &  \multicolumn{2}{c}{Topology-aware} & & iter.\ t.\\
\cmidrule{3-5}
\cmidrule{7-8}
\cmidrule{10-10}
Dataset &  Method & Corr. & Compl.  & Qual.&   &APLS & TLTS & & s\\
\cmidrule{1-10}
\multirow{4}{*}{\neurons}
&\baseline{}   &     97.2 &     94.0 &     91.5 &&     84.3 &     83.9 && 2.7 \\ 
&\snakeSimple{}&     97.4 &     95.2 &     92.9 &&     90.8 &     85.9 && 3.8 \\
&\snakeFast{}  &{\bf 97.0}&     {\bf 97.1} & {\bf 94.2} && 91.7& 88.1&& 5.3 \\
&\snakeFull{}  &     96.9 & 96.9& 94.1 && {\bf 91.8} &{\bf 89.3}&& 19.1\\
\cmidrule{1-10}
\multirow{4}{*}{\neuronsmisal{}}
&\baseline{}       &     82.1 &     86.5 &     72.8 &&     68.9 &     69.5 && 2.7 \\ 
&\snakeSimple{}&     83.2 &     87.7 &     74.5 &&     73.8 &     74.6 && 3.5 \\
&\snakeFast{}    &     84.2 &     {\bf 88.9}  &    {\bf 76.2} &&     {\bf 75.1} &  77.7 && 5.1 \\
&\snakeFull{}     &     {\bf 84.4}     &       88.5    &      76.1     &&      74.8     &      {\bf 78.1}     &&  18.9  \\
\cmidrule{1-10}

\multirow{4}{*}{\mra{}}
&\baseline{}       &     90.1     &     72.2     &     66.9     &&     49.8    &    50.4      && 2.8 \\ 
&\snakeSimple{}&     89.9     &     73.1      &     67.5     &&     53.5    &    53.1      && 3.7\\
&\snakeFast{}    & {\bf 90.3} & {\bf 73.5} &  {\bf 68.1} && {\bf 55.4} & {\bf 55.2} && 5.1\\
&\snakeFull{}     &       -        &       -        &       -        &&       -        &       -        && 18.5\\
\cmidrule{1-10}

\end{tabular}
\vspace{2mm}
\caption{
Performance of \DRU{} trained using Mean Squared Error \baseline{} and the proposed losses.
See section~\ref{subs:results} for a description.
 \label{tab:combined-dru}
}
 \vspace{-3mm}
\end{table}


==> tables/results_misaligned.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US
\begin{table}
\caption{
Performance of deep nets trained with different loss functions on the \neuronsmisal{} data set and the time needed for single training iteration.
%See section~\ref{subs:results} for description.
 \label{tab:results_misaligned}
}
\setlength{\tabcolsep}{3pt}
\center
\begin{tabular}{@{}l l  c c c  c c c  c  c c @{}}
\cmidrule{3-10}
 & & \multicolumn{3}{c}{Pixel-wise} & &  \multicolumn{2}{c}{Topology-aware} & & iter.\ t.\\
\cmidrule{3-5}
\cmidrule{7-8}
\cmidrule{10-10}
Arch. &  Method & Corr. & Compl.  & Qual.&   &APLS & TLTS & & s\\
\cmidrule{1-10}
\multirow{4}{*}{\UNet{}}
&\baseline{}       &     81.8     &     83.5     &     70.4     &&     65.8     &     63.6     && 2.8 \\ 
&\snakeSimple{}&     83.0     &     83.9     &     71.6     &&     70.4     &     68.8     && 3.4\\
&\snakeFast{}    &     83.1     & {\bf 85.5} &     72.9     &&     73.9     & {\bf 70.2} && 4.9\\
&\snakeFull{}     & {\bf 83.5} &     85.4     & {\bf 73.1} && {\bf 74.2} &    69.9      && 17.8\\
\cmidrule{1-10}
\multirow{4}{*}{\DRU{}}
&\baseline{}       &     82.1 &     86.5 &     72.8 &&     68.9 &     69.5 && 2.7 \\ 
&\snakeSimple{}&     83.2 &     87.7 &     74.5 &&     73.8 &     74.6 && 3.5 \\
&\snakeFast{}    &     84.2 &     {\bf 88.9}  &    {\bf 76.2} &&     {\bf 75.1} &  77.7 && 5.1 \\
&\snakeFull{}     &     {\bf 84.4}     &       88.5    &      76.1     &&      74.8     &      {\bf 78.1}     &&  18.3  \\
\cmidrule{1-10}
\end{tabular}
\end{table}


==> tables/results_mra.tex <==

% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{table}
\caption{
Performance of deep nets trained with our loss functions on the \mra{} data set and the time needed for single training iteration.
%See section~\ref{subs:results} for description.
 \label{tab:results_mra}
}
\setlength{\tabcolsep}{3pt}
\center
\begin{tabular}{@{}l l  c c c  c c c  c  c c @{}}
\cmidrule{3-10}
 & & \multicolumn{3}{c}{Pixel-wise} & &  \multicolumn{2}{c}{Topology-aware} & & iter.\ t.\\
\cmidrule{3-5}
\cmidrule{7-8}
\cmidrule{10-10}
Arch. &  Method & Corr. & Compl.  & Qual.&   &APLS & TLTS & & s\\
\cmidrule{1-10}
\multirow{4}{*}{\UNet{}}
&\baseline{}       &     90.1     &     72.2     &     66.9     &&     49.8    &    50.4      && 2.8 \\ 
&\snakeSimple{}&     89.9     &     73.1      &     67.5     &&     53.5    &    53.1      && 3.7\\
&\snakeFast{}    & {\bf 90.3} & {\bf 73.5} &  {\bf 68.1} &&     55.4    & {\bf 55.2} && 5.1\\
&\snakeFull{}     &     90.2     & {\bf 73.5} &     68.0     && {\bf 55.6} &    55.0      && 18.5\\
\cmidrule{1-10}
\multirow{4}{*}{\DRU{}}
&\baseline{}       &     80.2    &     79.3     &     66.3     &&     48.7      &    49.9      && 2.7 \\ 
&\snakeSimple{}&     80.7     &     79.9     &     67.1     &&    53.3      &    53.0      && 3.7\\
&\snakeFast{}    & {\bf 81.0} & {\bf 80.5} & {\bf 67.7} &&    55.3      & {\bf 55.4} && 5.2\\
&\snakeFull{}     &     80.9     & {\bf 80.5} &     67.6     && {\bf 55.6} &    55.2      && 18.8\\
\cmidrule{1-10}
\end{tabular}
\end{table}


==> tables/results_noise.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{table}
\caption{
Performance of \UNet{} trained using \snakeFast{} and \baseline{} on the \neurons{} data set with different annotation noise levels.
%See section~\ref{subs:results} for description.
 \label{tab:results_noise}
}
\setlength{\tabcolsep}{3pt}
\center
\begin{tabular}{@{}l l  c c c  c c c  c  c c @{}}
%\cmidrule{3-10}
 & & \multicolumn{3}{c}{Pixel-wise} & &  \multicolumn{2}{c}{Topology-aware} & & iter.\ t.\\
\cmidrule{3-5}
\cmidrule{7-8}
\cmidrule{10-10}
Noise &  Method & Corr. & Compl.  & Qual.&   &APLS & TLTS & & s\\
\cmidrule{1-10}
\rule{0pt}{0ex}
\multirow{2}{*}{{\it No Noise}}
&\baseline{}   & 98.9 & 91.3 &     90.4 &&     80.3 &     80.9 && 2.8 \\ 
&\snakeFast{}  & 98.7 & 95.0 &{\bf 93.8}&&{\bf 91.1}&{\bf 85.9}&& 5.2 \\
%\cmidrule{1-10}
\rule{0pt}{3ex}
\multirow{2}{*}{{\it Level 1}}
&\baseline{}   & 97.3 & 86.7 &     84.8 &&     71.8 &     70.5 && 2.8 \\ 
&\snakeFast{}  & 98.7 & 94.6 &{\bf 93.4}&&{\bf 87.4}&{\bf 83.2}&& 5.2 \\
%\cmidrule{1-10}
\rule{0pt}{3ex}
\multirow{2}{*}{{\it Level 2}}
&\baseline{}   & 42.7 & 38.5 &     25.6 &&     63.3 &     63.6 && 2.8 \\ 
&\snakeFast{}  & 92.1 & 84.9 &{\bf 79.2}&&{\bf 86.2}&{\bf 82.3}&& 5.2 \\
%\cmidrule{1-10}
\rule{0pt}{3ex}
\multirow{2}{*}{{\it Level 3}}
&\baseline{}   & 16.1 & 13.9 &      8.1 &&     55.4 &     53.7 && 2.8 \\ 
&\snakeFast{}  & 31.3 & 27.2 &{\bf 17.3}&&{\bf 79.8}&{\bf 76.8}&& 5.2 \\
\cmidrule{1-10}
\end{tabular}
\end{table}


==> tables/results_sota.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{table}
\caption{
Comparison to label correction methods on the \neurons{} and \neuronsmisal{} data sets.
%See section~\ref{subs:results} for description.
 \label{tab:results_sota}
}
\setlength{\tabcolsep}{3pt}
\center
\begin{tabular}{@{}l l  c c c  c c c  c  c c @{}}
\cmidrule{3-10}
 & & \multicolumn{3}{c}{Pixel-wise} & &  \multicolumn{2}{c}{Topology-aware} & & iter.\ t.\\
\cmidrule{3-5}
\cmidrule{7-8}
\cmidrule{10-10}
Data &  Method & Corr. & Compl.  & Qual.&   &APLS & TLTS & & s\\

\cmidrule{1-10}
\multirow{4}{*}{\neurons{}}
&\COPLE{}   &     97.7 &     97.0 &   {\bf 94.8}   &&     81.0 &     83.6 && 2.8 \\ 
&\QAM{}      &     94.5 &     {\bf 98.8} &     93.5 &&     87.3 &     84.5 && 4.2 \\ 
&\DS{}          &     97.5 &     97.0 &     {\bf 94.7} &&     83.8 &     84.1 && 5.8 \\ 
&\snakeFast{}  &       {\bf 98.7}     &  95.0 & 93.8 &&{\bf 91.1}&{\bf 85.9}&& 5.2 \\

\cmidrule{1-10}
\multirow{4}{*}{\neuronsmisal{}}
&\COPLE{}   &     85.2 &     83.4 &     {\bf 72.8} &&     67.6 &     65.2 && 2.8 \\ 
&\QAM{}      &     {\bf 89.8} &     79.3 &     {\bf 72.8} &&     71.2 &     68.6 && 4.2 \\ 
&\DS{}          &     83.2 &     81.6 &     70.0 &&     71.0 &     68.8 && 5.8 \\ 
&\snakeFast{}    &     83.1     & {\bf 85.5} &     {\bf 72.9}     &&     {\bf 73.9}     & {\bf 70.2} && 4.9\\

\cmidrule{1-10}
\multirow{4}{*}{\mra{}}
&\COPLE{}       &     85.5      &     77.3      &     {\bf 68.3}    &&     50.2     &     53.8      && 2.8 \\ 
&\QAM{}         &     80.2      &     80.1      &          66.8     &&     54.3     &     54.2      && 4.2 \\ 
&\DS{}          &     82.0      & {\bf 80.3}    &          68.1     &&     55.0     &     54.9      && 5.8 \\ 
&\snakeFast{}   & {\bf 90.3}    &     73.5      &          68.1     &&{\bf 55.4}    & {\bf 55.2}    && 5.1 \\

\cmidrule{1-10}
\end{tabular}
\end{table}


==> tex/method_old.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\section{Method}
\label{sec:method}

Given a set of microscopy stacks along with the corresponding and possibly imprecise centerline annotations, we want to train a deep net to produce precise delineation.
To that end, in each training iteration, we align the annotations with the predictions, and use these aligned centerline annotations to compute the loss function.
We first present the standard training procedure and explain why it is sub-optimal when the annotations lack precision. We then formalize the training procedure we designed to address this issue.

\subsection{Standard Training Procedure}
\label{sec:standard}

Let us consider a set of $N$ microscopy scans $\{\bX_i\}_{1 \leq i \leq N}$ and corresponding centerline annotations $\{\by_i\}_{1 \leq i \leq N}$, in the form of distance maps of the same size as the scans, that is, volume in which $\by[p]$ is the distance from voxel $p$ to the closest centerline voxel. Let  $F(\cdot;\Theta)$ be a deep network, with weights $\Theta$. We want to train it to take as input a scan $\bX$ and return a volume $F(\bX,\Theta)$, containing a delineation of centerlines visible in $\bX$. The traditional approach to learning the network weights is to make $F(\bX,\Theta)$ as close as possible to $\by$ by solving
%
\begin{equation}
\Theta^*=\argmin_{\Theta}  \sum_{i=1}^N L\big(\by_i,F(\bX_i;\Theta)\big) \;, \label{eq:standardObjective}
\end{equation}
%
where the loss term $L(\by,F(\bX;\Theta))$ is a function of the voxel-wise difference between the annotation and the prediction. This assumes that the deviations of the annotations from actual centerline trajectories are small and unbiased. In reality, they rarely are. Hence, the network learns to accommodate this uncertainty in the annotations by blurring the predictions. At test time, this leads to breaking the continuity of predictions wherever the image quality is compromised by high level of noise or low contrast between the foreground and the background.

%represented as binary volumes of the same size as the scans, where $\by[p]=1$ when the voxel $p$ is crossed by a centerline, and $\by[p]=0$ otherwise.

\subsection{Overview of our Approach}
\label{sec:proposed}

The formulation of Eq.~\ref{eq:standardObjective} assumes that the deviations of the annotations from reality are small and unbiased. This work is predicated on the fact that they rarely are and that we must allow for substantial deviations from the original annotations. 

Thus, instead of encoding the annotations in terms of volumes $\by_i$, we represent the annotated centerline $\mC_i$ of each $\bX_i$ as a graph with $n^v_i$ vertices connected by $n^e_i$ edges that represent short line segments, as shown in Fig.~\ref{fig:snake}. Let $\bc_i$ be the vector of dimension $3 n^v_i$ formed by concatenating the 3D coordinates of the vertices of $\mC_i$. For each $\bc_i$, we introduce a {\it deformation vector} $\bd\bc_i$ also of dimension $3 n^v_i$, that can be added to $\bc_i$. Doing so changes the shape of $\mC_i$ but preserves its topology and can be used to explicitly model the deviation of the annotated centerlines from their true position. In other words, the minimization problem can be reformulated as finding 
%
\begin{align}
\Theta^*,\bd\bC^*               & = \argmin_{\Theta,\bd\bC}  L_{\rm dat} (\Theta,\bd\bC)+ L_{\rm reg} (\bd\bC) \; ,  \label{eq:newObjective} \\
\mbox{where } L_{\rm dat} (\Theta,\bd\bC) &= \sum_{i=1}^N L\big(D(\bc_i+\bd\bc_i),F(\bX_i;\Theta)\big), \label{eq:extEnergy}
\end{align}
%
$\bd\bC$ is the vector obtained by concatenating all the $\bd\bc_i$, $D$ is a distance transform that creates a volume in which each voxel is assigned its truncated distance to the closest edge of $\mC$, and $L_{\rm reg}$ is a regularization term that forces the deformed centerlines to be smooth and not too distant from the original ones. 

Solving the problem of Eq.~\ref{eq:newObjective} means training the network to find centerlines that are smooth, not too far from the annotations, and with the same topology. This is what we want but, unfortunately, this optimization problem involves two kinds of variables, the components of $\bC$ and $\Theta$ respectively, which are not commensurate in any way. In practice, this makes optimization difficult. We address this problem by eliminating the $\bC$ variables by rewriting Eq.~\ref{eq:newObjective} as
%
\begin{align}
\bd\bC^*(\Theta)          & =  \argmin_{\bd\bC} L_{\rm dat} (\Theta,\bd\bC) + L_{\rm reg} (\bd\bC)    \;  \label{eq:defObjective}\; ,\\
\Theta^*                       & =  \argmin_{\Theta}  L_{\rm dat} (\Theta,\bd\bC^*(\Theta)) + L_{\rm reg} (\bd\bC^*(\Theta))\; .                        \label{eq:ourObjective}
\end{align}
%
In the following section, we will show that $\bd\bC^*(\Theta)$  can be approximated by a differentiable function of $\Theta$ whose derivatives we can express analytically. The optimization problem of Eq.~\ref{eq:ourObjective} has now become a standard differentiable optimization problem that we can solve using the usual tools of the trade. 

\subsection{Annotations as Network Snakes}
\label{sec:netsnakes}

We propose to represent each $\mC_i$ as a network snake~\cite{Fua96f,Butenuth12}, and to take $L_{\rm reg}$ to be a classical sum of spring and elasticity terms~\cite{Kass88}, that can be written as
%
\begin{align}
 L_{\rm reg} (\bd\bC) = \frac{1}{2} \sum_i (\bc_i + \bd\bc_i)^T A (\bc_i + \bd\bc_i) \; ,
 \end{align}
%
where $A$ is a very sparse matrix. Given this quadratic formulation of $L_{\rm reg}$, we can use the well-known semi-implicit scheme introduced to deform snakes, also known as active contour models~\cite{Kass88}, to minimize Eq.~\ref{eq:defObjective}. It involves first initializing the displacement of each snake to a vector of zeros $\bd\bc_i^0$ and refining it by iteratively solving
%
\begin{equation}
(\bA+\alpha \bI) (\bc_i+\bd\bc^{t+1}_i)=\alpha(\bc_i+\bd\bc^t_i)- \nabla L\big(D(\bc_i+\bd\bc_i^{t}),F(\bX_i;\Theta)\big)  \;, \label{eq:viscosity}
\end{equation}
%
for $\bd\bc^{t+1}_i$, consecutively for $0 \leq t < T$, where $T$ is a fixed number of iterations that is sufficient for the process to stabilize, typically 10 in our implementation. 
We take  $\bd\bC^*(\Theta)$ to be the concatenation  for all $i$ of the resulting vectors $\bc^T_i$.
When the iteration stabilizes, we have $\forall i, \bd\bc^{t}_i \approx \bd\bc^{t+1}_i$. Therefore we can substitute $\bd\bc^{t+1}_i$ by  $\bd\bc^{t}_i$ in Eq.~\ref{eq:viscosity}. This yields
%
\begin{align}
\forall i, 0 & \approx \bA (\bc_i+\bd\bc^t_i) + \nabla L\big(D(\bc_i+\bd\bc_i^{t}),F(\bX_i;\Theta)\big)  \; , \nonumber \\
\Rightarrow  0 &  \approx \frac{\partial L_{\rm reg}}{\partial \bd\bC}\big(\bd\bC^*(\Theta)\big) + \frac{\partial L_{\rm dat}} {\partial \bd\bC}\big(\Theta,\bd\bC^*(\Theta)\big)  \;  . \label{eq:zerograd} 
\end{align}
%
The right-hand-side of Eq.~\ref{eq:zerograd} is the gradient of the total loss function~\eqref{eq:defObjective} with respect to $\bd\bC$. In words, at $\bd\bC^*(\Theta)$, the gradient of the total loss function is almost zero, which means that $\bd\bC^*(\Theta)$ minimizes $L_{\rm reg}+L_{\rm dat}$ and is a solution of Eq.~\ref{eq:defObjective}. 

In practice, we solve Eq.~\ref{eq:viscosity} by inverting the matrix $(\bA+\alpha \bI)$ in the beginning of the training procedure, and multiplying the right-hand-side of the equation by the inverse in each iteration. 
%This lets us define $\bd\bC^*(\Theta)$ analytically as 
%\begin{equation}
%\bd\bc^{t+1}_i=(\bA+\alpha \bI)^{-1} \Big(\alpha(\bc_i+\bd\bc^t_i)- \nabla L\big(D(\bc_i+\bd\bc_i^{t}),F(\bX_i;\Theta)\big)\Big)-\bc_i  \;, \label{eq:update}
%\end{equation}

\subsection{Computing the Gradients of the Loss Function}

%\MK{It is true that we do not need to differentiate the snake with respect to $\Theta$, but only for the case when the snake energy is equal to the training objective. For our other case of the simple energy, we do need to backpropagate through snake updates. So, in this section, lets explain this basic case where they are equal, and let's leave the more complicated case for the next subsection.} \PF{Agreed.}

Performing the minimization in Eq.~\ref{eq:ourObjective} requires computing at each iteration the gradient of the loss with respect to $\Theta$, that is, 
%
\begin{multline}
\frac{\partial}{\partial \Theta} \Big(L_{\rm dat}\big(\Theta,\bd\bC^*\big)  + L_{\rm reg}\big(\bd\bC^*\big)\Big) =\\
\frac{\partial L_{\rm dat}}{\partial \Theta}(\Theta,\bd\bC^*) + 
\Big(\frac{\partial L_{\rm dat}}{\partial \bd\bC}(\Theta,\bd\bC^*)+\frac{\partial L_{\rm reg}}{\partial \bd\bC}(\bd\bC^*)\Big) \frac{\partial \bd\bC^*}{\partial \Theta}  \; , \label{eq:aux1}
\end{multline}
%
%where all the terms are evaluated with argument $\Theta$ and $\bd\bC^*(\Theta)$.
where we omitted the dependence of $\bd\bC^*$ on $\Theta$ for clarity.
By its definition in Eq.~\ref{eq:defObjective}, $\bd\bC^*$ approximates the minimum of $L_{\rm dat}+L_{\rm reg}$, so 
%
\begin{align}
   \frac{\partial L_{\rm dat}} {\partial \bd\bC}(\Theta,\bd\bC^*) +  \frac{\partial L_{\rm reg}}{\partial \bd\bC}(\bd\bC^*)\approx 0 \; .
\end{align}  
%
%as already noted in Eq.~\ref{eq:zerograd}. 
Hence, the second term of Eq.~\ref{eq:aux1} vanishes and we have
%
\begin{align}
	\frac{\partial}{
\partial\Theta} 
\Big(L_{\rm dat}\big(\Theta,\bd\bC^*\big)+ L_{\rm reg}\big(\bd\bC^*\big)\Big)
%}{\partial \Theta} 
&\approx  \frac{\partial L_{\rm dat}}{\partial \Theta}(\Theta,\bd\bC^*) \; .
\end{align}
%
\pf{Therefore, even though $\bC^*$ is a function of $\Theta$, we do {\it not} need to compute its derivatives with respect to $\Theta$ to perform backpropagation. We only need those of $L_{\rm dat}$ and can treat $\bC^*$ as a constant when evaluating them. We now turn to the training procedure, which exploits this important property of our loss function.}

\subsection{Training Scheme}
\label{sec:training}

Because computing the gradients of our loss function does not require computing the derivatives of the annotations locations with respect to network weights, we can implement the forward and backward steps required to perform back-propagation in three steps:
%
\begin{enumerate} 

\item Perform the forward pass as in any other network;

\item Compute $\bd\bC^*$ by iteratively solving Eq.~\ref{eq:viscosity} and update the annotations accordingly; 

\item Perform the backward pass, given the updated annotations. 

\end{enumerate}
%
We will refer to this approach as \snakeFull{}. \pf{It is depicted on the left side of Fig.~\ref{fig:grads}} and we will see in the results section that it performs well but is slow. Classical network snakes formulation~\cite{Fua96f,Butenuth12} were not subject to such a slowdown because their energy functions were easy to compute.  By contrast, computing our external energy $L_{\rm dat}$ of our snake~\eqref{eq:extEnergy} requires computing the distance from each pixel to each snake edge and doing this repeatedly is computationally demanding. 

\input{fig/training}

To alleviate this problem, we introduce a second approach that we will refer to as  \snakeFast{}. Let $L_{\rm snake}$ be the classical external snake energy~\cite{Kass88} that can be written as a sum of image values at each snake vertex
%
\begin{equation}
L_{\rm snake}(\bc;\Theta)=\sum_{k} \big(F(\bX;\Theta)*G\big)[c_k],
\end{equation}
%
where $*G$ denotes a convolution with a Gaussian kernel and $F()[c_k]$ denotes the network output at vertex $c_k$. It is much faster to compute than $L_{\rm dat}$ but, in practice, minimizing it yields very similar results in which the  snake vertices slide towards image where the $F(\bX;\Theta)$ is small. We can therefore replace $L_{\rm dat}$  by  $L_{\rm snake}$ in Eq.~\ref{eq:defObjective} and iteratively solve
%
\begin{align}
\bd\bC^{\dagger}(\Theta)          & =  \argmin_{\bd\bC} L_{\rm snake} (\Theta,\bd\bC) + L_{\rm reg} (\bd\bC)    \;  \label{eq:snakeFunc}\; , \\
\Theta^*                       & =  \argmin_{\Theta}  L_{\rm dat} (\Theta,\bd\bC^\dagger(\Theta)) \; , \label{eq:ourObjective2}
\end{align}
%
instead of Eqs,~\ref{eq:defObjective} and Eqs.~\ref{eq:ourObjective}. The gradient of the loss becomes 
%
\begin{multline}
\frac{\partial}{\partial \Theta} \Big(L_{\rm dat}\big(\Theta,\bd\bC^\dagger\big)  + L_{\rm reg}\big(\bd\bC^\dagger\big)\Big) =\\
\frac{\partial L_{\rm dat}}{\partial \Theta}(\Theta,\bd\bC^\dagger) + 
\Big(\frac{\partial L_{\rm dat}}{\partial \bd\bC}(\Theta,\bd\bC^\dagger)+\frac{\partial L_{\rm reg}}{\partial \bd\bC}(\bd\bC^\dagger)\Big) \frac{\partial \bd\bC^\dagger}{\partial \Theta}  \; , \label{eq:aux2}
\end{multline}
%
where the first term is the same gradient of the loss with respect to the network parameters given $\bd\bC^\dagger$ as before and computing the second term requires backpropagation through the snake 
update procedure of~\ref{sec:netsnakes}. Fortunately, this can this can be done easily because the snake update~\eqref{eq:viscosity} is a linear map. \PF{You could elaborate a little on that. It is not obvious to non-initiated. Also, is that why you do a fixed number of update iterations? That should be said somewhere. } This approach is illustrated in Fig.~\ref{fig:grads}.

In section~\ref{sec:experiments}, we analyze the time and accuracy tradeoffs between \snakeFull{}  and \snakeFast{}. Somewhat surprisingly, the latter is not only faster but also tends to yields better training results, which we will discuss there. \PF{True?} 

\comment{
Our formulation may be extended to compute $\bd\bC^*$ in another way, and it works as long as $\bd\bC^*$ can be differentiated with respect to $F()$.
This may be indicated when running the snake with a complex external energy function $L_{\rm dat}$ turns out to be too slow.
In our experiments, we consider a simple alternative external energy formulation for the snake
%
\begin{equation}
E_\text{ext}\big(\bc,F(\bX;\Theta)\big)=\sum_{0<p\le n^v} F(\bX;\Theta)[\bc_p] \;, \label{eq:ext1}
\end{equation}
%
where $\bc_p$ is the position of the $p$-th node of the delineation $\bc$ and by $F[v]$ we denote the value of volume $F$ at position $v$.
This energy makes the snake nodes slide into regions where the prediction $F(\bX;\Theta)$ is low.
Its advantage is that it is simple and fast to compute.

In this case, the gradient is composed of two terms,
%
\begin{equation}
\frac{\partial}{\partial \Theta} L\big(R(\bc^*_i),\by \big) = 
(\frac{\partial}{\partial R }L() \frac{\partial}{\partial \bc} R() \frac{\partial}{\partial \by} \bc^*+ \frac{\partial}{\partial \by} L())
\end{equation}
%
where the first terms corresponds to the backpropagation through the snake update procedure, and the second term is the customary gradient of the loss with respect to the prediction.
A priori, it is not clear if it should be used when external energy of type~\eqref{eq:ext1} is adopted: the gradient tends to make the network output more suited for making the snake converge, but does not make the prediction more similar to the ground truth.
We will answer this question experimentally.
}

\subsection{Architecture and Loss Terms}

To implement the network $F$ of Section~\ref{eq:formal}, we use a U-Net architecture~\cite{Ronneberger15} that we train to estimate the distance function to the closest annotation. In this section, we first describe the loss function $L$ of Eq.~\ref{eq:standardObjective} we use for this purpose and then the regularizer $R$ of Eq.~\ref{eq:newObjective}.

\paragraph{\bf Loss Function $L$.}

As a centerline estimate $\mC$ with vertices $\by$ defines continuous contours connecting its vertices, we can compute the distance function $D_i(\by_i)$ that it  induces. \PF{The formal definition belongs here along with the proof that it can be differentiated with respect to both sides.} 

We can then take $L$ to be 
%
\begin{equation}
L\big(\by_i,F(\bX_i;\Theta)\big) =  \|F(x_i;\Theta) - \min(d,D_i(\by)) \|^2 \; ,
\end{equation}
%
where $d$ is a value with use to truncate $D$. \PF{Why? And why do you use the $l^2$ norm?}. In practice, we use $d=20$. \PF{20 what? And why?}



